MegBA: A GPU-Based Distributed Library for Large-Scale Bundle Adjustment

Large-scale Bundle Adjustment (BA) requires massive memory and computation resources which are difficult to be fulfilled by existing BA libraries. In this paper, we propose MegBA, a GPU-based distributed BA library. MegBA can provide massive aggregated memory by automatically partitioning large BA problems, and assigning the solvers of sub-problems to parallel nodes. The parallel solvers adopt distributed Precondition Conjugate Gradient and distributed Schur Elimination, so that an effective solution, which can match the precision of those computed by a single node, can be efficiently computed. To accelerate BA computation, we implement end-to-end BA computation using high-performance primitives available on commodity GPUs. MegBA exposes easy-to-use APIs that are compatible with existing popular BA libraries. Experiments show that MegBA can significantly outperform state-of-the-art BA libraries: Ceres (41.45$\times$), RootBA (64.576$\times$) and DeepLM (6.769$\times$) in several large-scale BA benchmarks. The code of MegBA is available at https://github.com/MegviiRobot/MegBA.

==> table/one_step.tex <==
\begin{table*}[ht!]
\centering
\begin{tabular}{l|l|l|l|l|l|l}

& Venice-52 & Venice-245 & Venice-1778 & Ladybug-1031 & Trafalgar-257 & Dubrovnik-356 \\
\hline
Squared Error & 3.4e5   & 1.1e6     & 1.8e6     & 3.0e5      & 1.6e5       & 7.9e5      \\
\hline
DeepLM(FP64) & 0.334 & 0.611 & 3.352 & 0.290 & 0.342 & 0.956 \\
\hline
MegBA-1(FP32) & \textbf{0.0196}    & \textbf{0.035}      & \textbf{0.160}       & Failed       & \textbf{0.011}         & \textbf{0.044}         \\ 
\hline
MegBA-1(FP64) & 0.228     & 0.389      & 1.404      & \textbf{0.072}        & 0.087         & 0.313
\end{tabular}
\caption{\textbf{Performance of One Update Step.} \textit{We test DeepLM on precision FP64 and MegBA on precision FP32 and FP64 with one GPU. The table shows the time that different algorithms consumed for a single BA update step.}}

\label{tab:one_step}
\end{table*}

==> table/sota.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Library} &
  \textbf{Automatic Differentiation} &
  \textbf{Construction of the Hessian w/o explicit parameter blocks} &
  \textbf{GPU Support} &
  \textbf{Distributed} &
  \textbf{No need for other algorithms to distribute} &
  \textbf{Exact Distributed Solution} &
  \textbf{High Performance} &
  \textbf{Can solve general BA problems} &
  \textbf{Test on extreme large-scale datasets} \\ \hline
Ceres  & {\color[HTML]{202124} Yes} & No   & No                         & No & N.A. & N.A. & No                         & {\color[HTML]{202124} Yes} & No \\ \hline
g2o    & {\color[HTML]{202124} Yes} & No   & No                         & No & N.A. & N.A. & No                         & {\color[HTML]{202124} Yes} & No \\ \hline
PBA    & N.G.                       & No   & {\color[HTML]{202124} Yes} & No & N.A  & N.A  & Depends                    & {\color[HTML]{202124} Yes} & No \\ \hline
IPU    & No                         & N.G. & No                         & No & N.A. & N.A. & {\color[HTML]{202124} Yes} & N.G.                       & No \\ \hline
Disney & N.G.                       & N.G. & {\color[HTML]{202124} Yes} & No & N.A. & No   & {\color[HTML]{202124} Yes} & No                         & No \\ \hline
RPBA   & N.G.                       &      &                            &    & No   & No   &                            &                            &    \\ \hline
DPBA   & N.G.                       &      &                            &    &      &      &                            &                            &    \\ \hline
STBA   & N.G.                       &      &                            &    & No   & No   &                            &                            &    \\ \hline
DeepLM &                            &      &                            &    &      &      &                            &                            &    \\ \hline
MegaBA &
  {\color[HTML]{202124} Yes} &
  {\color[HTML]{202124} Yes} &
  {\color[HTML]{202124} Yes} &
  {\color[HTML]{202124} Yes} &
  {\color[HTML]{202124} Yes} &
  {\color[HTML]{202124} Yes} &
  {\color[HTML]{202124} Yes} &
  {\color[HTML]{202124} Yes} &
  {\color[HTML]{202124} Yes} \\ \hline
\end{tabular}%
}

\caption{\textbf{Summary of the Bundle Adjustment Libraries} }
\label{tab:sota_compare}
\end{table*}


%\caption{\textbf{Summary of the Bundle Adjustment Libraries} }
% \label{tab:sota_compare}
